Representational Alignment Across Model Layers and Brain Regions with Multi-Level Optimal Transport

Standard representational similarity methods align each layer of a network to its best match in another independently, producing asymmetric results, lacking a global alignment score, and struggling with networks of different depths. These limitations arise from ignoring global activation structure and restricting mappings to rigid one-to-one layer correspondences. We propose Multi-Level Optimal Transport (MOT), a unified framework that jointly infers soft, globally consistent layer-to-layer couplings and neuron-level transport plans. MOT allows source neurons to distribute mass across multiple target layers while minimizing total transport cost under marginal constraints. This yields both a single alignment score for the entire network comparison and a soft transport plan that naturally handles depth mismatches through mass distribution. We evaluate MOT on vision models, large language models, and human visual cortex recordings. Across all domains, MOT matches or surpasses standard pairwise matching in alignment quality. Moreover, it reveals smooth, fine-grained hierarchical correspondences: early layers map to early layers, deeper layers maintain relative positions, and depth mismatches are resolved by distributing representations across multiple layers. These structured patterns emerge naturally from global optimization without being imposed, yet are absent in greedy layer-wise methods. MOT thus enables richer, more interpretable comparisons between representations, particularly when networks differ in architecture or depth. We further extend our method to a three-level MOT framework, providing a proof-of-concept alignment of two networks across their training trajectories and demonstrating that MOT uncovers checkpoint-wise correspondences missed by greedy layer-wise matching.

==> iclr2026/extras.tex <==

\section{Background and Motivation}

A common strategy for comparing two pretrained networks is to align their layers in a \emph{pairwise} fashion.  Concretely, given two models with hidden‐activation matrices
\[
X_\ell \in \mathbb{R}^{T\times n_\ell},\quad
Y_m \in \mathbb{R}^{T\times n'_m},
\]
one computes for each source layer \(\ell\) the target layer
\[
m^*(\ell)
\;=\;\arg\min_{m}\;W_2^2\bigl(\mathcal{U}(X_\ell),\,\mathcal{U}(Y_m)\bigr),
\]
where \(W_2^2\) is the squared‐Wasserstein distance between the empirical measures \(\mathcal{U}(X_\ell)\) and \(\mathcal{U}(Y_m)\).  A neuron–to–neuron transport plan \(Q_{\ell m^*(\ell)}\) is then computed via
\[
Q_{\ell m^*}
\;=\;\arg\min_{Q\in U(n_\ell,n'_{m^*})}
\sum_{i,j}Q_{ij}\,\|X_\ell(i)-Y_{m^*}(j)\|^2.
\]
Although simple, this \emph{pairwise} approach has two major drawbacks:
\begin{itemize}
  \item \textbf{Depth mismatch:}  If the two networks have different numbers of layers, neurons in one layer may naturally align to neurons spread across several layers of the other network.  A hard one‐to‐one choice \(m^*(\ell)\) cannot capture such cross‐depth relationships.
  \item \textbf{Lack of global consistency:}  Each layer match is chosen independently, ignoring information from all other layers.  This greedy selection can overfit to noise in the activations of a single layer.
\end{itemize}

\section{Hierarchical Optimal Transport Alignment}

To address these issues we propose a \emph{hierarchical} optimal transport formulation.  Let
\[
\{X_1,\dots,X_L\},\;\{Y_1,\dots,Y_M\}
\]
be the activations of the two networks.  We introduce:
\begin{itemize}
  \item \emph{Inner plans} \(Q_{\ell m}\in U(n_\ell,n'_m)\), the neuron‐to‐neuron couplings between layer \(\ell\) and layer \(m\).
  \item \emph{Outer plan} \(P\in U(L,M)\), the layer‐to‐layer coupling matrix.
\end{itemize}
We solve
\[
\min_{P\in U(L,M),\;\{Q_{\ell m}\}}
\sum_{\ell=1}^L
\sum_{m=1}^M
P_{\ell m}\,
\underbrace{W_2^2\bigl(\mathcal{U}(X_\ell),\mathcal{U}(Y_m)\bigr)}_{=\,\min_{Q_{\ell m}}\sum_{i,j}Q_{ij}\,\|X_\ell(i)\!-\!Y_m(j)\|^2}
\]
where each inner cost is itself a Wasserstein‐2 problem.  In practice, we:
\begin{enumerate}
  \item Compute all neuron plans
    \[
    Q_{\ell m}
    = \arg\min_{Q\in U(n_\ell,n'_m)}
      \sum_{i,j}Q_{ij}\,\|X_\ell(i)-Y_m(j)\|^2
    \quad\text{and}\quad
    C_{\ell m} \;=\;\text{EMD}_2^2(X_\ell,Y_m).
    \]
  \item Solve the \emph{outer} transport
    \[
    P
    = \arg\min_{P\in U(L,M)}
      \sum_{\ell,m}P_{\ell m}\,C_{\ell m}.
    \]
\end{enumerate}

The resulting \(P\) is a \emph{soft} matching of layers that enforces global consistency via the marginal constraints
\[
\sum_m P_{\ell m} = \tfrac1L, 
\quad
\sum_\ell P_{\ell m} = \tfrac1M,
\quad
P_{\ell m}\ge0.
\]
Rather than committing each source layer \(\ell\) to a single target layer, the hierarchical plan allows a neuron in layer \(\ell\) to distribute its mass across multiple layers \(m\), naturally handling networks of differing depths.

\section{Global Neuron–to–Neuron Plan}

From the computed \(\{P,Q\}\) one can assemble a single “global” coupling
\[
G\in\mathbb{R}^{\bigl(\sum_\ell n_\ell\bigr)\times\bigl(\sum_m n'_m\bigr)},
\]
by placing each block
\[
G_{[\,\ell,m\,]}
=\;P_{\ell m}\;Q_{\ell m}
\]
into the rows corresponding to layer \(\ell\) and columns corresponding to layer \(m\).  This matrix \(G\) aligns \emph{every} neuron in one network to \emph{every} neuron in the other, respecting both the local activation geometry and the global layer‐matching constraints.
